Learning as Conversation: Dialogue Systems Reinforced for Information Acquisition

We propose novel AI-empowered chat bots for learning as conversation where a user does not read a passage but gains information and knowledge through conversation with a teacher bot. Our information-acquisition-oriented dialogue system employs a novel adaptation of reinforced self-play so that the system can be transferred to various domains without in-domain dialogue data, and can carry out conversations both informative and attentive to users. Our extensive subjective and objective evaluations on three large public data corpora demonstrate the effectiveness of our system to deliver knowledge-intensive and attentive conversations and help end users substantially gain knowledge without reading passages. Our code and datasets are publicly available for follow-up research.

==> Learning as conversation/2_sec_approach.tex <==


\section{Approach}


In order to obtain an informative and attentive teaching dialogue system, we propose a framework that consists of two chat bots in different roles, and leverage both supervised learning and unsupervised reinforcement learning, as illustrated in Figure~\ref{fig:frame}. The unsupervised reinforcement learning enables the system to be fine-tuned on other text corpus where no annotation or dialogue data is required.

\begin{figure}[H]
\centering
\includegraphics[width=3.0in]{Learning as conversation/imgs/framework.drawio.png}
\caption{Our two-phase training framework}
\label{fig:frame}
\end{figure}




\subsection{Model Architecture}

Given a passage $P$, the conversation between Teacher bot $X$ and Student bot $Y$ can be denoted as a sequence 
of turns $C = \{U_1^X, U_1^Y, ..., U_{N}^X, U_{N}^Y\}$, where $N$ is the number of turns in the conversation. 
 In order to mimic our use case, Teacher bot has access to $P$ whereas Student bot does not.

\textbf{Teacher bot $X$} aims at transmitting the information in $P$ to the student. 
At the $n_{th}$ turn, $X$ takes as input $P$ and
the conversation history $H_n^Y =\{U_1^X, U_1^Y, ..., U_{n-1}^X, U_{n-1}^Y\}$, and outputs $U_{n}^X$.
Teacher bot $X$ adopts DoHA~\cite{prabhumoye-etal-2021-focused}, a pre-trained model for document-grounded text generation, and is tuned in supervised phase and unsupervised self-play phase.

In order to fine-tune Teacher bot $X$ with reinforcement learning on full conversations, 
as a practical approach, we train a
\textbf{Student bot $Y$} to carry on conversations with $X$. 
Student bot $Y$ takes the conversation history $H_n^Y =\{U_1^X, U_1^Y, ..., U_{n}^X\}$ as input, 
and output $U_{n}^Y$.
It adopts BART~\cite{lewis-etal-2020-bart} model.

\subsection{Phase 1: Supervised Pre-Tuning}

This phase trains Teacher bot $X$ to initialize and carry out conversations based on a given passage $P$, and trains Student bot $Y$ to respond appropriately to $X$. 
To this end, we pre-tune both $X$ and $Y$ on the  \textsl{Wizard of Wikipedia} (\textsl{WoW}) dataset. \textsl{WoW} was chosen as the pre-tuning dataset because of its two characteristics: 1) Open-domain: \textsl{WoW} contains conversations on a broad range of topics and domains across Wikipedia, thus the pre-tuned Teacher and Student bots have greater potentials to be successfully transferred to other domains during the fine-tuning stage; 2) Content-grounded: in \textsl{WoW}, the teaching bot's utterances are grounded on passages, which is similar to our task. 
We present the gold passage to Teacher bot directly, though, different from the \textsl{WoW}'s original setting~\cite{dinan2019wizard} where Teacher bot searches a large corpus for supporting passages. 



We optimize the maximum-likelihood objective for Teacher bot by minimizing the following loss:
{\medmuskip=1mu
\thinmuskip=1mu
\thickmuskip=1mu
\nulldelimiterspace=0pt
\scriptspace=0pt
\begin{align*}
L_{mle}^X = -\sum_{n=1}^N\sum_{m=1}^{M_n}log(p(x_{m}|x_{1}, ..., x_{m-1}, H_n^X, P))
\end{align*}}

\noindent where $N$ is the total number of turns in the conversation, $\{x_1, ..., x_{M_n}\}$ is Teacher bot's response at the $n_{th}$ turn, ${M_n}$ is the number of words in $U^X_n$.
The loss function for Student bot, $L_{mle}^Y$, is similar to $L_{mle}^X$, with the exception of not including a passage $P$ as input.
\begin{align*}
L_{mle}^Y = -\sum_{n=1}^N\sum_{m=1}^{M_n}log(p(y_{m}|y_{1}, ..., y_{m-1},  H_{n}^Y))
\label{equ: lms}
\end{align*}

\noindent where $\{y_1, ..., y_{M_n}\}$ is Student bot's response at the $n_{th}$ turn.

\subsection{Phase 2: Unsupervised Self-Play Fine-tuning}
\label{Sec: usp}

In this phase, we aim at improving Teacher bot's ability to present informative and coherent conversations. 
This is achieved by reinforcement learning on Teacher bot with the help of Student bot, and could be applied in a novel target domain even where dialogue dataset is absent.
We adopt a self-play approach, i.e. we let Teacher bot and Student bot chat with each other over a passage in the target domain to generate multiple turns of conversations. In this fine-tuning phase, we keep Student bot frozen, and reward Teacher bot when the generated conversation achieves higher scores.
%\footnote{In the fine-tuning phase we only optimize Teacher bot, and keep Student bot frozen}.  
In order to reduce the variance of the gradient estimate, we apply self-critic reinforcement learning~\cite{Rennie2017cvpr}.
Specifically, at each turn, we let Teacher bot generate two separate utterances: 1) $U^s$, which is sampled from the model, i.e. $x_{m}^s\sim p(x|x_{1}^s, ..., x_{m-1}^s)$, and 2) $U^*$, which is obtained by greedy search, i.e. $x_m^* = \argmax_w p(x|x_{1}^*, ..., x_{m-1}^*)$.
We optimize the model by minimizing the following RL loss:
\begin{align*}
L_{rl}^X = -\sum_{n=1}^N( R(U^s_n) - R(U^*_n) )\sum_{m=1}^{M_n} log(p(x^s_{m}\\|x^s_{1}, ..., x^s_{m-1},  H_{n}^X, P))
\end{align*}

\noindent where $R()$ is the reward function, which we will cover in Section~\ref{Sec:rl}, and $P$ is a passage from the target domain corpus. 

If not taking into account language modeling, optimizing RL loss alone would lead Teacher bot to generate inarticulate and even grammatically incorrect utterances. 
To keep the fluency of Teacher bots, we optimize a combined loss $L^X$ consisting of RL loss $L_{rl}^X$ on the new target domain data and MLE loss $L_{mle}^X$ on the pre-tuning dialogue dataset, so the language style acquired during the pre-tuning phase would not get lost during RL fine-tuning:
\begin{align*}
L^X = \gamma L_{rl}^X + (1-\gamma)L_{mle}^X
\end{align*}

\noindent where $\gamma\in(0,1)$ is a scaling factor accounting for the emphasis on $L_{rl}^X$ and $L_{mle}^X$. 
We note that 
while $L_{mle}^X$ should be obtained on an annotated content-grounded dialogue dataset (e.g. \textsl{WoW}), $L_{rl}^X$ could be obtained on any target domain passage corpus even without dialogue data. This enables our approach to be transferred to an unsupervised text corpus. 




\subsection{Reward Functions}
\label{Sec:rl}

\subsubsection{Coverage}

We define the coverage reward of a Teacher bot's utterance $U^X$ as: 
\begin{align*}
R_{cov} = \textsc{Rouge}_1(P, H + U^X) - \textsc{Rouge}_1(P, H)
\end{align*}

\noindent where $\text{Rouge}_1(P, H)$ is the Rouge-1 F1~\cite{lin-2004-rouge} score of the conversation history $H$ to the input passage $P$. Intuitively, this function favors utterances that cover more information in the passage and have less overlap with the conversation history. 

\subsubsection{Coherence}
\label{sec: coh}

\begin{description}[style=unboxed,leftmargin=0cm]
\item[Dialogue coherence datasets]
We explore neural coherence scoring models trained on two open-domain dialogue coherence datasets: 

1. \textsl{WoW-coherence dataset} \quad
We reuse the \textsl{WoW} dataset to heuristically build a dialogue coherence classification dataset. Specifically, for each multi-turn dialogue in \textsl{WoW}, we label the ground truth response to its conversation history as \emph{coherent} response, and all later responses in the same dialogue as \emph{incoherent} responses. 

2. \textsl{InferConv dataset}~\cite{dziri-etal-2019-evaluating} \quad
This is an open-domain dialogue coherence classification dataset built from PersonaChat conversational data~\cite{zhang-etal-2018-personalizing}.
The dataset casts a response as the hypothesis and the conversation history as the premise, thus convert dialogue coherence evaluation into an NLI task. 
The dataset classifies the relationship between the response and the conversation history into three categories: \emph{entailed}, \emph{neutral} and \emph{contradict}.
Table~\ref{Tab:sta2} summarizes statistics of these datasets. 

\item[Coherence scoring models]
Based on the same pre-trained model BERT~\cite{devlin-etal-2019-bert}, we train two different coherence scoring models on the two dialogue coherence classification datasets respectively. 
Both models take the concatenation (with [SEP]) of the conversation history and a candidate response as input, 
and minimize the cross entropy loss between the predicted label and the gold label. 
We use different methods to attain the coherence reward $R_{coh}$ from the two models. 


For model \textsl{WoW-coherence}, we define the coherence reward with softmax: 
\[R_{coh} = \frac{e^{o_c}}{e^{o_c} + e^{o_i}}\]
 where $o_c$ and $o_i$ are the logits for \emph{coherent} and \emph{incoherent} labels in the output layer. 
For model \textsl{InferConv}, 
we observe some responses labeled as \emph{neutral} are appropriate responses but are not closely related to conversation history (e.g. \emph{``That's interesting!''}),
 we thus heuristically assign constant scores $s_e$, $s_n$ and $s_c$ as coherence reward $R_{coh}$ when the response is predicted as \emph{entailed}, \emph{neutral} and \emph{contradict}.
In the remainder of the paper, we use \textsl{WoW-coherence} as the default coherence model, and compare it with \textsl{InferConv} in Section~\ref{sec:obj_results}.

\end{description}

\subsubsection{Mixed Reward}

The coverage and coherence rewards are combined with a hyper-parameter $\beta$, yielding the final reward:
\begin{align*}
    R = \beta R_{cov} + (1-\beta)R_{coh} 
\end{align*}




==> Learning as conversation/3_sec_exps.tex <==
\section{Experimental Settings}
\label{sec:settings}

We proceed by describing our datasets, comparison systems and evaluation metrics.
We then show the performance of our proposed approach compared to state-of-the-art in \S\ref{sec:obj_results}.

\subsection{Datasets}
\label{sec:datasets}


\textsl{Wizard of Wikipedia}~\cite{dinan2019wizard} contains a total of 22,311 human-human conversations crowdsourced via Amazon's Mechanical Turk. 
The conversations are grounded in Wikipedia passages covering a wide range of topics: \emph{e-book}, \emph{toga party}, \emph{armadillo}, etc. 
Both Teacher and Student bots are pre-tuned on the \textsl{WoW} dataset during Phase 1.
Different from \textsl{WoW}'s original setting,
we present the gold passage to the Teacher bot directly,
instead of searching a large corpus for supporting passages. 
This allows us to focus less on retrieval and more on creating a Teacher bot to deliver informative and attentive dialogues.

We consider knowledge sources of various sorts as Teacher bot's target domain during fine-tuning. 
CNN/DailyMail contains a large collection of online news articles with an average of 781 tokens per article~\cite{see-etal-2017-get}. 
The full content of the article cannot be conveyed in a short conversation. 
Thus, we use the first 130 tokens of each article as a supporting passage, assuming it covers the most important content of the news article. 


Academic papers have become an omnipresent source of knowledge.
We create our own dataset containing papers published in recent years (2017--2021) 
at major venues, including ACL, EMNLP, NAACL, EACL, Findings and ICLR conferences.
Similarly, we use paper abstracts as supporting passages instead of full articles. 
Moreover, we include Wikipedia passages from the \textsl{WoW} dataset, without conversations, as another source of knowledge.
The \textsl{CNN-DM}, \textsl{Paper Abstracts} and \textsl{Wikipedia} datasets are used in Phase 2 of unsupervised self-play fine-tuning.  
Statistics of these datasets are summarized in Table~\ref{Tab:sta1}.

\begin{table}[t]
% \begin{center}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.05}
\footnotesize
\centering
\begin{tabular}{|p{2.3cm}rrr|}
\hline
\rowcolor{gray!10}
\textbf{Pre-Tuning} & \multicolumn{2}{r}{\textsl{WoW-Train}} & \textsl{WoW-Valid} \\
\#Utterances & \multicolumn{2}{r}{166,787} & 17,715 \\
\#Dialogues & \multicolumn{2}{r}{18,430} & 1,948  \\
\#Words/utterance & \multicolumn{2}{r}{16.6} & 16.6  \\
\#Words/passage & \multicolumn{2}{r}{110.3} & 109.8 \\
\hline
\hline
\rowcolor{gray!10}
\textbf{Fine-Tuning} & \textsl{Wikipedia} & \textsl{CNN-DM} & \textsl{Paper Abs.}  \\
\#Passages        & 50,000   & 50,000   & 22,512  \\
\#Words/passage & 111.7    & 129.8    & 149.3  \\
\hline
\hline
\rowcolor{gray!10}
\textbf{Test Set} & \textsl{Wikipedia} & \textsl{CNN-DM} & \textsl{Paper Abs.}  \\
\#Passages            &  1,000    &  1,000    &  500      \\
\#Words/passage     &  112.7   &  129.9   &  148.1   \\
\hline
\end{tabular}
\caption{Datasets statistics.}
\label{Tab:sta1}
\end{table}

\begin{table}[t]
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.05}
\footnotesize
\begin{tabular}{|p{1.46cm}rrrr|} 
\hline
\rowcolor{gray!10}
\textbf{WoW-Coh}  & \multicolumn{2}{r}{\textsl{Coherent Resp.}} & \textsl{Incoherent} & \textsl{All} \\
Train & \multicolumn{2}{r}{74,092} & 233,142       & 307,234 \\
Valid & \multicolumn{2}{r}{3,939} & 12,362        & 16,301  \\
Test & \multicolumn{2}{r}{3,865} & 12,098        & 15,963  \\
\hline
\hline
\rowcolor{gray!10}
\textbf{InferConv} & \textsl{Entail} & \textsl{Neutral} & \textsl{Contradict} & \textsl{All}\\
Train & 218,181 & 579,434 & 261,984 & 1,059,599\\
Valid & 28,072 & 12,242 & 9,780 & 50,094\\
Test & 3,119 & 1,087 & 1,360 & 5,566\\
\hline
\end{tabular}
\caption{Details of the datasets used to train our neural coherence scoring models.}
\label{Tab:sta2}
\vspace{-0.1in}
\end{table}



\begin{table}[t]
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\centering
\begin{scriptsize}
\begin{fontppl}
\begin{tabular}{lp{7cm}}
\toprule
\multicolumn{2}{l}{\textbf{Coherence}}\\
3 & TeacherBot provides coherent responses to the evaluator's input. \\
2 & TeacherBot provides largely coherent responses (with minor coherency issues) to the evaluator's input.  \\
1 & TeacherBot does not respond properly to the evaluator's input. \\
\midrule
\multicolumn{2}{l}{\textbf{Readability}}\\
3 & TeacherBot's responses are easy to read, containing no grammatical or semantic errors. \\
2 & TeacherBot's responses read smoothly but may contain 1-2 grammatical or semantic errors. \\
1 & TeacherBot's responses contain >2 grammatical or semantic errors, or are nonsensical.  \\
\midrule
\multicolumn{2}{l}{\textbf{Overall Quality}}\\
\multicolumn{2}{p{7.3cm}}{An initial score of 3 is given to a dialogue, then 1 point is deducted for each of the following issues, with a minimum score of 0.} \\
$\bullet$ & Uninformative, i.e. it provides <2 correct answers during QA. \\
$\bullet$ & Incoherent, i.e. the average coherence score is <2 points. \\
$\bullet$ & Low readability, i.e. the average readability score is <2.5 points. \\
$\bullet$ & Any other issues that could lead to an ineffective conversation e.g. words are repeated between turns. \\
\bottomrule
\end{tabular}
\end{fontppl}
\end{scriptsize}
\vspace{-0.05in}
\caption{
A scoring rubric provided to human evaluators.
}
\label{Tab:hum_score}
\vspace{-0.15in}
\end{table}

\begin{table*}[ht!]
\setlength{\tabcolsep}{4.5pt}
\renewcommand{\arraystretch}{1.05}
\begin{center}
\scriptsize
\begin{tabular}{| l | c | c c c | c c | c c c | c | c | c | c | c |} 
\hline
\multirow{2}{*}{\textbf{Dataset}}  & \multirow{2}{*}{\textbf{Model}}  & \multicolumn{5}{c|}{\textbf{Coverage Metrics}} & \multicolumn{3}{c|}{\textbf{Coherence Metrics}} & \multicolumn{4}{c|}{\textbf{Subjective Metrics}} & \multirow{2}{*}{Avg Len}  \\
\cline{3-14}
& & R-1  & R-2   & R-L   & QA$_{\textsc{Conf}}$   & QA$_{\textsc{F1}}$ & WoW-Coh & InferConv & DPR$_{\textsc{Relv}}$ &  QA$_{\textsc{Human}}$  & Coh & Read & Overall &  \\
\hline
\multirow{4}{*}{\textbf{Wikipedia}}     
 & \textsc{DoHA}    & 48.09 & 41.27 & 44.31 & 19.76 & 19.39 & 0.503 & 0.550 & 0.555 &  30.0 & 2.07 & 2.79 & 1.84 & 15.51 \\
 & \textsc{+Cov}  & \textbf{74.62} & \textbf{71.66} & \textbf{72.25} & \textbf{30.90} & \textbf{34.38} & 0.307 & 0.466 & 0.543  & \textbf{45.63} & 1.85 & 2.85 & 2.12 & 28.11 \\
 & \textsc{+Coh}  & 44.87 & 35.87 & 39.64 & 18.96 & 17.17 & \textbf{0.807} & \textbf{0.694} & \textbf{0.578} &  33.12 & \textbf{2.42} & 2.81 & 2.34  & 17.11\\
 & \textsc{Full}      & 62.78 & 58.83 & 60.61 & 25.94 & 27.01 & 0.617 & 0.630 & 0.556 & 38.74 & 2.26 & \textbf{2.88} & \textbf{2.37} & 20.69 \\
\hline
\multirow{4}{*}{\textbf{CNN-DM}}     
 & \textsc{DoHA}     & 38.89  & 30.09 & 32.91 & 15.90 & 15.80 & 0.521 &  0.567 & 0.538 & 28.12 & 2.28 & 2.67 & 1.87 & 16.29 \\
 & \textsc{+Cov}  & \textbf{81.52} & \textbf{78.52} & \textbf{73.73} & \textbf{30.98} & \textbf{38.46} &  0.253 & 0.381 & 0.525 & \textbf{58.59} & 2.14 & \textbf{2.79} & 2.37 & 36.08 \\
 &\textsc{+Coh}  & 30.45 & 18.61 & 24.0  & 13.31 & 11.31 & \textbf{0.845} & \textbf{0.692} & \textbf{0.561} & 40.15 & 2.40 & 2.48 & 1.93 & 16.23 \\
 & \textsc{Full}     & 65.77 & 60.45 & 57.83 & 25.5 & 30.36 & 0.604 & 0.692 & 0.559  & 52.5 & \textbf{2.57} & 2.71 & \textbf{2.53} & 29.76 \\
\hline
\multirow{4}{*}{\textbf{Papers}}     
& \textsc{DoHA}     & 36.27 & 28.20 & 30.60 & 10.29 & 5.34  & 0.565 & 0.452  & 0.557 & 30.5 & 1.58 & 2.55 & 1.4 & 15.61 \\
& \textsc{+Cov}  & \textbf{72.63} & \textbf{69.69} & \textbf{49.18} & \textbf{20.32} & \textbf{17.61}  & 0.271 & 0.141 & 0.529 & \textbf{57.5} & 1.73 & \textbf{2.77} & 1.96 & 33.55 \\
& \textsc{+Coh}  & 32.96 & 21.24 & 26.21 & 8.18  & 3.95  & \textbf{0.806}  & \textbf{0.547} & \textbf{0.576} & 25.47 & 1.82 & 2.26 & 1.25 & 16.3 \\
& \textsc{Full}      & 59.65 & 54.22 & 47.88 & 15.46 & 13.81 & 0.766 & 0.501 & 0.560 &  51.76 & \textbf{2.16} & 2.53 & \textbf{2.09} & 27.37 \\
\hline
\end{tabular}
\caption{
% Evaluation results of models fine-tuned on each dataset. 
We compare Teacher bots based on naive DoHA\cite{prabhumoye-etal-2021-focused} model to variants fine-tuned using different reward functions, Avg len refers to average utterance length.}
\label{Tab:obj}
\end{center}
\vspace{-0.1in}
\end{table*} 


\subsection{Comparison Models}
\label{sec:baselines}

Our baseline Teacher bot builds on the state-of-the art content-grounded dialogue generation model: \textsc{DoHA}~\cite{prabhumoye-etal-2021-focused}. 
It includes two improvements to the architectures of pre-trained encoder-decoder models~\cite{lewis-etal-2020-bart}: building context-driven representation of the supporting document, and enabling document-headed attention to acquire information from the document. 
\textsc{DoHA} has demonstrated strong performance in document-grounded generation. 
All \textsc{DoHA} models are pre-tuned on the \textsl{WoW} dataset.

Our \textsc{Full}  Teacher bot is created to converse in an informative and coherent manner. 
It extends \textsc{DoHA} by incorporating both coverage and coherence rewards in unsupervised self-play fine-tuning.
Additionally, we ablate \textsc{Full} model by removing each of the two rewards:
\textsc{+Cov} uses only the coverage reward for fine-tuning, i.e. setting $\beta=1$ in our reward function (\S\ref{Sec:rl}).
\textsc{+Coh} utilizes only the \textsl{WoW-coherence} reward, i.e. setting $\beta=0$.
Please refer to \hyperref[sec:appendix]{appendix} for
more implementation details and hyper-parameters.


\subsection{Evaluation Metrics}

We investigate a wide range of metrics to evaluate Teacher bot's performance.
\textsl{Objective metrics} measure the content coverage and coherence of Teacher bot's utterances.
\textsl{Subjective metrics}, devised with human-in-the-loop, provide a holistic evaluation of a conversation, focusing on its overall effectiveness and various aspects of linguistic quality. 

\begin{description}[style=unboxed,leftmargin=0cm]
\item[Objective Metrics.]
Teacher bot converses with Student bot over a passage for three turns.
That is, Teacher bot initiates the dialogue and provides two responses to Student bot. 
We objectively evaluate Teacher bot's utterances in terms of information coverage and coherence as follows. 



\begin{itemize}[style=unboxed,leftmargin=0cm]
    \item 
\textsc{Rouge}~\cite{lin-2004-rouge} is one of the most widely used metrics for measuring information coverage.
We consider three variants in this study: \textsc{R-1}, \textsc{R-2} and \textsc{R-L}, which respectively measure the overlap of unigrams, bigrams and the longest common subsequence between  the given passage and Teacher bot's utterances.

\item  \textsl{QA}$_{\textsc{F1}}$ and \textsl{QA}$_{\textsc{Conf}}$ are two variants of 
SummaQA~\cite{scialom-etal-2019-answers}, a question answering-based evaluation metric.
If a conversation is rich in information, it could be used as a surrogate for the passage to answering important questions. 
To this end,
SummaQA generates Cloze-style questions from a passage by masking out entities, 
then employs a QA system to answer those questions based on a conversation. 
A higher QA performance suggests the conversation has better coverage. 
Particularly, \textsl{QA}$_{\textsc{F1}}$ reports the F1 score for question answering;
\textsl{QA}$_{\textsc{Conf}}$ measures the confidence of the QA system in predicting answers. 

\item  \textsl{WoW-Coherence} and \textsl{InferConv} are neural coherence scoring models (\S\ref{sec: coh}) repurposed for evaluation. 
These models quantitatively assess if Teacher bot has produced a coherent response given the conversation history, or not. 

\item \textsl{DPR$_{\textsc{Relv}}$} provides a new perspective on dialogue coherence evaluation~\cite{zhang2018reinforcing}.
It draws on the Dense Passage Retriever model (DPR; Karpukhin et al., 2020)\nocite{karpukhin-etal-2020-dense}
to predict if a Teacher bot's response is relevant to Student bot's input.
A higher relevance score means the input and response share the same topic, 
suggesting a coherent conversation.

\end{itemize}


\item[Subjective Metrics.]
We recruit 24 human evaluators to interact with Teacher bots. 
Each evaluator is asked to converse with bots over four passages. 
For each passage, the evaluator chats with four different Teacher bots for three turns,
where Teacher bot initiates the conversation and responds twice to the evaluator's input.
We randomly select 48 passages for evaluation, i.e., 16 passages from each of the three test sets.
To evaluate conversations produced from \textsl{Paper Abstracts}, we require evaluators, 8 in total, to be either PhD students or have obtained a PhD degree. 
For fair comparison, we shuffle and hide the order of Teacher bots presented to evaluators. 
Human evaluators were suggested to feed the same or similar inputs across Teacher bots on the same passage whenever possible. 
Throughout the conversation, the passage was not shown to the evaluators. 
After the conversation, human evaluators were asked to complete the following evaluation tasks: 

\begin{itemize}[style=unboxed,leftmargin=0cm]
\item \textsl{QA}$_{\textsc{Human}}$: 
Five sentences are randomly selected from each passage and one important entity is masked out in each sentence. The evaluators are presented with each corrupted sentence and asked if the sentence could be recovered by referencing the conversation with Teacher bot. We report the ratio of sentences that could be correctly recovered. 

\item \textsl{Linguistic Quality}: We ask human evaluators to rate each conversation along three dimensions: 
\emph{Coherence}: Does Teacher bot provide coherent responses to the evaluator's input?  
\emph{Readability}: Are Teacher bot's utterances easy to read, containing no grammatical or semantic errors?
\emph{Overall Quality}: How will the conversation score in terms of informativeness, coherence, readability and all aspects considered?
The scoring rubric provided to human evaluators is shown in Table~\ref{Tab:hum_score}.


\end{itemize}

\end{description}




==> Learning as conversation/4_sec_objective.tex <==


\section{Objective Results}
\label{sec:obj_results}



\begin{description}[style=unboxed,leftmargin=0cm]
\item[Results on Test Sets.]
Table~\ref{Tab:obj} presents objective evaluation results obtained for various Teacher bots on three test sets: \textsl{CNN-DM}, \textsl{Paper Abstracts} and \textsl{Wikipedia}.
We observe that our \textsc{Full} Teacher bot is able to substantially outperform the baseline system \textsc{DoHA} on all datasets and across all objective metrics.  
It strikes a fine balance between delivering information-rich conversations and ensuring those conversations are coherent and attentive.  
Further, we find that optimizing a single reward, whether it be coverage or coherence, produces suboptimal results. 
For instance, \textsc{+Cov} tends to produce longer utterances than other variants. 
It improves information coverage, but yields low coherence scores,
leading to a performance even inferior to the baseline \textsc{DoHA}.
Our findings suggest that it is important for the reinforcer $L_{rl}^X$ to learn with both coverage or coherence rewards.




\begin{figure}[t]
\centering
\includegraphics[width=3.1in]{imgs/rouge_gain_1.8.5.pdf}
\caption{ROUGE gain and utterance length tend to decrease as the number of turns increases}
\label{Fig: gain}
\end{figure}


\item[Trading off Coverage for Coherence.]
In Figure~\ref{Fig: finetune_scores}, we plot the learning curves of coverage and coherence scores when the reinforcer adopts a single reward (\textsc{+Cov}, \textsc{+Coh}) or both (\textsc{Full}). 
We use $R_{cov}$ and $R_{coh}$ to approximate coverage and coherence scores.
These plots are generated using 50 validation instances from the \textsl{Paper Abstracts} dataset.
We observe that with only the coverage reward (\textsc{+Cov}), Teacher bot tends to aggressively copy content from the passage, while disregarding the conversation history. 
This inevitably leads to incoherent conversations.
Conversely, \textsc{+Coh} can improve on coherence, but falls short on delivering informative conversations. 
Finally, our \textsc{Full} Teacher bot trades off coverage for substantially higher coherence, thus achieving a significant improvement over the baseline \textsc{DoHA} model.


\begin{figure*}
\centering
\includegraphics[width=5.5in]{imgs/scores_new.pdf}
\caption{Coverage and coherence scores when applying different reward scores}
\label{Fig: finetune_scores}
\end{figure*}

\item[Trading off Coverage for Coherence.]
We are curious to know the amount of information brought by each utterance produced by Teacher bot.  
To this end, we define information gain $\mathcal{IG}(\cdot)$ as the improvement of ROUGE scores brought by an utterance $U$:
\begin{align*}
\mathcal{IG}(U) = 
\textsc{Rouge}(P, H+U) - \textsc{Rouge}(P, H),
\end{align*}

\noindent where $P$ is the supporting passage, and $H$ represents the conversation history.
We consider three \textsc{Rouge} variants, \textsc{R-1}, \textsc{R-2} and \textsc{R-L}, respectively.
Figure~\ref{Fig: gain} illustrates the gain of information for each of the three turns.
The average \textsc{Rouge} gain is reported for each turn, using conversations produced for the \textsl{Paper Abstracts} dataset. 
We observe that there is a general tendency across turns that information gain is decreasing. 
This is in part because that at the beginning of a conversation, Teacher bot has no constraints regarding content selection, it could rephrase any content selected from the supporting passage to initiate a dialogue. 
In subsequent turns, Teacher bot has to exercise caution in response generation considering both the conversation history and overall coherence of the conversation. 
Consequently, we find that the average length of the utterances also decreases in subsequent turns. 



\begin{table}[t]
\setlength{\tabcolsep}{4.5pt}
\renewcommand{\arraystretch}{1.05}
\begin{center}
\scriptsize
\begin{tabular}{| l | c | c c | c c c |} 
\hline
\multirow{2}{*}{\textbf{Dataset}}  & \multirow{2}{*}{\textbf{Model}}  & \multicolumn{2}{c|}{\textbf{Coverage}} & \multicolumn{3}{c|}{\textbf{Coherence}}  \\
\cline{3-7}
& & \textsl{QA}$_{\textsc{Conf}}$ & \textsl{QA}$_{\textsc{F1}}$ & WoW-Coh & IC & DPR  \\
\hline
\multirow{2}{*}{\textbf{Wikipedia}}     
& \textsl{WoW}  & 18.96 & 17.17 & \textbf{0.807} & \textbf{0.694} & \textbf{0.578} \\
& \textsl{InferCov}   & 20.41 & 19.61 & 0.647  & 0.676  & 0.561 \\
\hline
\multirow{2}{*}{\textbf{CNN-DM}}     
& \textsl{WoW}  & 13.31 & 11.31  & \textbf{0.845} & 0.692 & \textbf{0.561} \\
& \textsl{InferCov}   & 14.95 & 14.07  & 0.719 & \textbf{0.728} & 0.550 \\
\hline
\multirow{2}{*}{\textbf{Papers}}     
& \textsl{WoW}  & 8.18  &  3.95 & \textbf{0.806} & 0.547 & \textbf{0.576} \\
& \textsl{InferCov}   & 9.47  &  4.31 & 0.737 & \textbf{0.554} & 0.558 \\
\hline
\end{tabular}
\caption{Teacher bot's performance when using different coherence score models during fine-tuning}
\label{Tab:obj-coh}
\end{center}
\vspace{-0.1in}
\end{table} 


\item[A Comparison of Coherence Scoring Models.]
We compare two Teacher bots fine-tuned only with coherence reward from different coherence scoring models (i.e. \textsl{WoW-coherence} and \textsl{InferConv}). We demonstrate their objective results in Table~\ref{Tab:obj-coh}. According to the results,  Teacher bot fine-tuned with \textsl{InferConv} achieves slightly better coverage metrics. However, in terms of coherence metrics, Teacher bot fine-tuned with \textsl{WoW-coherence} model generally achieves better performance. Based on this observation, \textsl{WoW-coherence} scoring model better measures coherence in conversations.

\end{description}


==> Learning as conversation/5_sec_subjective.tex <==
\section{Subjective Results}



We demonstrate the subjective evaluation results in Table~\ref{Tab:obj} and have the following observations: 
\begin{enumerate}[style=unboxed,leftmargin=0cm]
    \item 
 For question answering, \textsc{+Cov} achieves the best performance on all three datasets. This again proves that the coverage reward helps make the conversation more informative;

\item For coherence scores, \textsc{+Coh} achieves the best performance on \textsl{Wikipedia}. However, on the other two datasets it was outperformed by \textsc{Full}. 

\item For readability scores, on \textsl{CNN-DM} and \textsl{Paper Abstracts}, \textsc{+Coh} achieves the lowest performance while \textsc{+Cov} achieves the highest.  

\item For overall scores, \textsc{Full} demonstrates the best performance. This suggests \textsc{Full} delivers conversations that are more balanced in coverage, coherence and readability. 

\item The \textsl{Paper Abstracts} corpus is the most challenging among all the test corpora, as our Teacher bots generally show worse performance in coherence, readability and overall scores. We found passages in \textsl{Paper Abstracts} contain volumes of professional vocabularies thus are more complicated for people to understand. In addition, it's also more difficult for Student bot to respond appropriately during self-play fine-tuning (See examples in \hyperref[sec:appendix]{appendix}). As a result, transferring Teacher bots to this domain is more challenging.

\end{enumerate}



\begin{table}[h]
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\centering
\begin{scriptsize}
\begin{fontppl}
\begin{tabular}{l p{6.5cm}}
\toprule[2pt]
\multicolumn{2}{c}{\textbf{Example A} (Passage from \textsl{Wikipedia})}\\
\midrule
\rowcolor{Gray}{\textbf{Passage}} & The Concorde is a British–French turbojet-powered supersonic passenger airliner ... It had a maximum speed over twice the speed of sound, at Mach 2.04, ... First flown in 1969, Concorde entered service in 1976 and operated for 27 years. ... \\
{\textbf{User}} & What is the plane famous for? \\

\rowcolor{Gray}{\textbf{Bot Cov}} &  First flown in 1969, Concorde entered service in 1976 and operated for 27 years.  \\

{\textbf{Bot Coh}}&   Concorde is famous for \underline{the speed of sound} at Mach 2.04. \\

\rowcolor{Gray}{\textbf{Bot Full}}&  Concorde is famous for having a maximum speed over twice the speed of sound, at Mach 2.04. \\
\midrule

\multicolumn{2}{c}{\textbf{Example B} (Passage from \textsl{CNN News})}\\
\midrule
\rowcolor{Gray}{\textbf{Passage}} & The US Food and Drug Administration, ... Molnupiravir is for the treatment of mild-to-moderate coronavirus disease in adults with positive results of direct SARS-CoV-2 viral testing ... This is the second Covid-19 antiviral pill authorized for ill people to take at home, before they get sick enough to be hospitalized ... \\

{\textbf{User}} & Tell me more about the drug. \\


\rowcolor{Gray}{\textbf{Bot Cov}}  & This is the second Covid-19 antiviral pill authorized for ill people to take at home, before they get sick enough to be hospitalized.  \\

{\textbf{Bot Coh}}& The drug is for people with mild to moderate coronavirus disease. \\

\rowcolor{Gray}{\textbf{Bot Full}}& Molnupiravir is for the treatment of mild-to moderate coronavirus disease in adults with positive results of direct SARS-CoV-2 viral testing. \\
\midrule

\multicolumn{2}{c}{\textbf{Example C} (Passage from \textsl{Paper Abstracts})}\\
\midrule
\rowcolor{Gray}{\textbf{Passage}} &  ... In this paper we describe a novel framework to guide a supervised, extractive summarization system with question-answering rewards ... Our results compare favorably with those reported by strong summarization baselines as evaluated by automatic metrics and human assessors ... \\
{\textbf{User}} & What did you propose? \\

\rowcolor{Gray}{\textbf{Bot Cov}} &  Our results compare favorably with those reported by strong summarization baselines as evaluated by automatic metrics and human assessors.  \\

{\textbf{Bot Coh}}&  A proposal to use the extractive summarizer \underline{to answer questions.} \\

\rowcolor{Gray}{\textbf{Bot Full}}& We propose a novel framework to guide a supervised, extractive summarization system with question-answering rewards. \\
\bottomrule[2pt]
\end{tabular}
\end{fontppl}
\end{scriptsize}
\vspace{-0.05in}
\caption{A few example responses from different Teacher bots. 
In example A,\textsc{+Coh} and \textsc{Full} abstractively generates \emph{Concord is famous for ...} to make the response more coherent to user's question. However, the \underline{underlined part} in \textsc{+Coh}'s statement misrepresent the input passage and is inaccurate.
In example B, all responses seem coherent because of the open-ended question.
}
\label{Tab:case}
\vspace{-0.15in}
\end{table}




\begin{description}[style=unboxed,leftmargin=0cm]
\item[A Case Study.]

\noindent We show a few Teacher bots' responses to users in Table~\ref{Tab:case}. After analyzing the cases, we have the following observations: 
\begin{enumerate}[style=unboxed,leftmargin=0cm]
    \item 
The coverage reward encourages Teacher bots to directly copy content from the input passage, while the coherence reward encourages  abstractively generating new content: As shown in Example A, \textsc{+Cov} directly extracts a part of the original passage as response, regardless of the user's question, while \textsc{+Coh} and \textsc{Full} abstractively rewrite the response to make it more coherent. 

\item
Putting too much weight on coherence reward could make Teacher bot become so abstractive that it misrepresents the original passage and lead to incoherence and semantic/grammar errors. (See \textsc{+Coh}'s response in example A and C) This explains \textsc{+Coh}'s low coherence and readability scores on \textsl{CNN-DM} and \textsl{Paper Abstracts}. This observation suggests the necessity to carefully choose the weight for coherence rewards, and to coupling coherence reward with coverage reward, which could make the chat bot less abstractive. 

\item
Generally, user utterances could be classified into two categories: \textbf{Information-seeking queries}  which request certain information (e.g. the user's utterance in example A); \textbf{Open statements} which do not have specific requests (e.g. the user's utterance in example B). We found evaluators tend to give high coherence scores to response to open statements, as they could be addressed by a wider range of responses.

\end{enumerate}


\end{description}





































==> Learning as conversation/6_sec_related.tex <==
\section{Related Work}

\begin{description}[style=unboxed,leftmargin=0cm]
\item[Content-Grounded Dialogue Generation]
Content grounded dialogue generation is the task of using the information provided in external content (e.g. a passage, etc.) to guide dialogue generation. 

Compared to previous research, our task has the following novelties.
1) Compared to content-grounded information-retrieval-oriented dialogue such as doc2dial~\cite{, feng-etal-2020-doc2dial} and ABCD~\cite{chen-etal-2021-action} where the chat bot responds to user query in a passive way, we expect our chat bots to convey knowledge proactively. 
2) Compared to chit chat-oriented dialogue such as~\cite{zhou-etal-2018-dataset, dinan2019wizard, blenderbot1Komeili, blenderbot2Xu}, our task is more focused on extensive conversation in a particular topic, and aims at helping the end user acquire knowledge or information from a given passage. 
3) Contrasted to chat bots that are applied in a single domain~\cite{zhou-etal-2018-dataset, moghe-etal-2018-towards, xu2019review}, our chat bot could be transferred to other domains through self-talk based fine-tuning. 

Another line of research works focus on content grounded text generation models~\cite{prabhumoye-etal-2021-focused, Zhao2020Low-Resource}. Compared with ordinary text generation models (e.g. BART~\cite{lewis-etal-2020-bart}), these models are specifically designed to model external content as an additional input, and achieve better performance on content grounded dialogue generation tasks including \textsl{CMU DoG}~\cite{Zhao2020Low-Resource} and \textsl{Wizard of  Wikipedia}~\cite{dinan2019wizard}. 


\item[RL in Text Generation]
Reinforcement learning has been applied in various natural language generation tasks, including image caption~\cite{Rennie2017cvpr}, automatic summarization~\cite{paulus2018a}, machine translation~\cite{kang-etal-2020-dynamic} and poem generation~\cite{yang-etal-2019-generating}. Specifically, when applying reinforcement learning in dialogue generation~\cite{li-etal-2016-deep, zhao-etal-2019-rethinking, shi-etal-2019-build, yamazaki-aizawa-2021-phrase, liu-etal-2020-impress}, self-play is often used to enable scoring multi-turn dialogues.
Compared to previous dialogue generation research using RL and self-play, our two-phase framework enables transferring the teacher bot to other domains by optimizing a mixed reward of coverage and coherence. 


\item[Educational Dialogue Systems and Conversational QA]

There have been research works applying dialogue systems for educational purposes.
Some chat bots are for language practice.~\cite{Ruan2021EnglishBotAA, Stewart2007chat, Huang2017chat}
Others are specially designed for education in a single domain or task, e.g. moral education~\cite{peng2019task}, educational debate~\cite{yuan2008human}. Compared with previous educational dialogue systems, our system is for information acquisition without domain restriction. 
Our task is also related to conversational question answering (CQA), e.g.~\cite{kocisky-etal-2018-narrativeqa, rajpurkar2016squad, joshi2017triviaqa, zellers-etal-2018-swag}. However, most existing CQA systems passively response to user queries in single turn conversations, while our system actively engage with users in multi-turn conversations. 

\end{description}


